Local Independence Testing for Point Processes

Constraint based causal structure learning for point processes require empirical tests of local independence. Existing tests require strong model assumptions, e.g. that the true data generating model is a Hawkes process with no latent confounders. Even when restricting attention to Hawkes processes, latent confounders are a major technical difficulty because a marginalized process will generally not be a Hawkes process itself. We introduce an expansion similar to Volterra expansions as a tool to represent marginalized intensities. Our main theoretical result is that such expansions can approximate the true marginalized intensity arbitrarily well. Based on this we propose a test of local independence and investigate its properties in real and simulated data.

==> commands.tex <==
\newcommand{\dd}{\,\textrm{d}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\F}{\mathcal{F}}

\newcommand{\nikolaj}[1]{{\color{red}{\scriptsize NT:}#1}}
\newcommand{\niels}[1]{{\color{blue}{\scriptsize NRH:}#1}}

% Dummy overwrite
\newcommand{\autocite}[1]{#1}

% Colors used in ggplot and local independence graph
\definecolor{ggplot1}{RGB}{27,158,119}
\definecolor{ggplot2}{RGB}{217,95,2}
\definecolor{ggplot3}{RGB}{117,112,179}
\definecolor{ggplot4}{RGB}{231,41,138}

==> figures/fig-neurons-node-layout.tex <==
    \node (B0) at (0, 3)  {$N^0$};
    \node (B1) at (1, 2)  {$N^1$};
    \node (B2) at (1, 1)  {$N^2$};
    \node (B3) at (0, 0)  {$N^3$};
    \node (B4) at (-1, 1) {$N^4$};
    \node (B5) at (-1, 2) {$N^5$};
    %%%%
    \node (C0) at (3, 3){$N^0$};
    \node (C1) at (4, 2){$N^1$};
    \node (C2) at (4, 1){$N^2$};
    \node (C3) at (3, 0){$N^3$};
    \node (C4) at (2, 1) {$N^4$};
    \node (C5) at (2, 2) {$N^5$};
    %%%%
    \node at (0, -0.5) {First};
    \node at (3, -0.5) {Second};

==> packages.tex <==
\usepackage{cite}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage[T1]{fontenc}
\usepackage{latexsym}
\usepackage{mathrsfs}
\usepackage{tikz}
\usepackage{hyperref}
\usepgflibrary{arrows}
\usetikzlibrary{matrix,arrows,calc}
\usepackage{xcolor}

\DeclareMathOperator*{\argmin}{arg\,min}

% Enable multiplots
\usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
\usepackage{subfiles}
\usepackage[capitalize]{cleveref}

% Nice tables
\usepackage{booktabs}

% Theorems
\newtheorem{thm}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{lem}{Lemma}
\newtheorem{dfn}{Definition}
\newtheorem{cor}{Corollary}
\newtheorem{ass}{Assumption}

\theoremstyle{definition}
\newtheorem{ex}{Example}
\newtheorem{rem}{Remark}
\newtheorem{adv}{Math Box}
\newtheorem{rbox}{R Box}
\newtheorem{alg}{Algorithm}
\newtheorem{exer}{Question}
